Scalable Discrete-to-Continuous Channel Simulation for Compression and Privacy

Channel simulation has recently emerged as a useful component in machine learning systems where samples from a prescribed probability distribution are to be compressed. Yet, general channel simulation algorithms often suffer from high computational costs, random stopping times or, in the worst case, can require generating an infinite number of shared random samples. We introduce a scheme for both exact and approximate simulation of discrete-to-continuous channels which conversely uses a fixed number of random samples, and therefore has a runtime independent of the channel and the input. Unlike existing channel simulation schemes which generate a sequence of independent samples from a proposal distribution, our approach generates one sample, or alternatively a fixed number of samples, from each potential target distribution. We then apply a latent permutation to the samples before performing sample selection using an exponential race. Our scheme provides a flexible tradeoff between the number of generated samples and the compression rate. Using polar and multilevel coding, we scale our approach to handle long blocklengths in $O(n \log n)$ time in order to benefit from reduced per-symbol overhead. We conclude by demonstrating applications to variable-rate compression with stochastic VQ-VAEs and communication-efficient differentially private distributed mean estimation via exact simulation of the Gaussian mechanism.

==> sec/sec_lower_bound_proof.tex <==
The cost of transmitting any message $M$ with shared randomness $W$ is bound below by
\begin{IEEEeqnarray}{c}
    H(M \mid W) \geq H(M \mid W) - H(M \mid X, W) = I(X; M \mid W).
\end{IEEEeqnarray}
Since $W$ is generated independent of the input $X$,
\begin{IEEEeqnarray}{c}
    I(X; M \mid W) = I(X; M \mid W) + I(X; W) = I(X; M, W).
\end{IEEEeqnarray}
Since the decoder outputs $Y$ as a function of $M$ and $W$, adding $Y$ does not change the mutual information.
We get
\begin{IEEEeqnarray}{rCl}
    I(X; M, W) & = & I(X; M, W, Y) \\
    & = & I(X;Y) + I(X; W \mid Y) + I(X; M \mid Y, W) \\
    & \geq & I(X;Y) + I(X; W \mid Y).
\end{IEEEeqnarray}
Finally,
\begin{IEEEeqnarray}{c}
    \E[\ell(M)] \geq H(M \mid W) \geq I(X; Y) + I(X; W \mid Y).
\end{IEEEeqnarray}
For the permuted scheme in particular, the shared randomness comprises $\bar{U}^N$, $S^N$ and $\Pi$.
Substituting for $W$ gives 
\begin{IEEEeqnarray}{c}
    \E[\ell(M)] \geq I(X;Y) + I(X; \bar{U}^N, S^N, \Pi \mid Y) \geq I(X;Y) + I(X; \bar{U}^N \mid Y).
\end{IEEEeqnarray}
which is the desired lower bound.
We can also express this as
\begin{IEEEeqnarray}{rCl}
    I(X;Y) + I(X;\bar{U}^N \mid Y) & = & H(X) - H(X \mid Y) + H(X \mid Y) - H(X \mid Y, \bar{U}^N) \label{eqn:y_to_k_start} \\
    & \stackrel{\text{(a)}}{=} & H(X \mid \bar{U}^N) - H(X \mid Y, \bar{U}^N) \\
    & = & I(X; Y \mid \bar{U}^N) \\
    & \stackrel{\text{(b)}}{=} & I(X; K \mid \bar{U}^N) \label{eqn:y_to_k_end}
\end{IEEEeqnarray}
where in (a) we have used the fact that $\bar{U}^N$ is generated independently of $X$, and in (b) we have noticed that given the set of samples $\bar{U}^N$, the index $K$ uniquely determines $Y$ as a discrete choice from among them.
Similarly, as our setting assumes a continuous output distribution, knowing $Y$ also fully determines $K$ given $\bar{U}^N$. \hfill \IEEEQED{}

